A General Graph Spectral Wavelet Convolution via Chebyshev Order Decomposition

Spectral graph convolution, an important tool of data filtering on graphs, relies on two essential decisions: selecting spectral bases for signal transformation and parameterizing the kernel for frequency analysis. While recent techniques mainly focus on standard Fourier transform and vector-valued spectral functions, they fall short in flexibility to model signal distributions over large spatial ranges, and capacity of spectral function. In this paper, we present a novel wavelet-based graph convolution network, namely WaveGC, which integrates multi-resolution spectral bases and a matrix-valued filter kernel. Theoretically, we establish that WaveGC can effectively capture and decouple short-range and long-range information, providing superior filtering flexibility, surpassing existing graph wavelet neural networks. To instantiate WaveGC, we introduce a novel technique for learning general graph wavelets by separately combining odd and even terms of Chebyshev polynomials. This approach strictly satisfies wavelet admissibility criteria. Our numerical experiments showcase the consistent improvements in both short-range and long-range tasks. This underscores the effectiveness of the proposed model in handling different scenarios. Our code is available at https://github.com/liun-online/WaveGC.

==> sec/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As shown in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the computational efficiency of the proposed algorithms and how they scale with dataset size in section~\ref{conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clarify the assumption for main Theorem~\ref{cc} in Assumption~\ref{assumption}, and detialed proof is given in Appendix~\ref{all proof}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the new graph convolution architecture in section~\ref{methoddddd}, and give the hyperparameters in Table~\ref{para_1}. We also release part of code in~\url{https://anonymous.4open.science/r/WaveGC}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code and data for this paper can be accessed through~\url{https://anonymous.4open.science/r/WaveGC}.
\item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
\item[] Justification: As shown in Appendix~\ref{ajsoifbfnd}, experiment settings.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: But we report the standard deviation of the mean for main results in section~\ref{saeaseasesaeasease}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The information for computer resources are reported in Appendix~\ref{Operating environment}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work is a foundational research on graph convolution and not tied to particular applications. We do not foresee any direct impacts on the society.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code and data for this paper can be accessed through~\url{https://anonymous.4open.science/r/WaveGC}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sec/sec_limitation.tex <==
\section{Limitation}
One potential limitation of \M\ is the computational complexity. The main contribution of \M\ is to address long-range interactions in graph convolution, so it inevitably establishes connections between most of nodes. This results in the same $O(N^2)$ complexity as Transformer~\cite{va_trans} and Specformer~\cite{specformer}. A possible solution is to decrease the number of considered frequency modes from $N$ to $\nu$. In this way, the complexity is reduced to $O(\nu\cdot N)$. This operation makes \M\ run on large-scale graph, i.e. \texttt{ogbn-arxiv}, and the best performance supports this simplification. Future work will focus on further simplification and scaling up to larger graphs.

==> sec/sec_theorem_.tex <==
\section{From Graph Convolution to Graph Wavelets}
In this section, our objective is to introduce a novel framework for learning expressive graph wavelet representations through convolution operations. We refer to this model as \M\ and demonstrate its theoretical flexibility in capturing both local and global information.

\subsection{Spectral Graph Convolution}
Spectral graph convolution is a fundamental operation in the field of graph signal processing~\cite{shuman2013emerging}. Specifically, given a signal matrix (or node features) $\bm{X}\in\mathbb{R}^{N\times d}$ on graph $\mathcal{G}$, the spectral filtering of this signal is defined with a kernel $\bm{\kappa}\in\mathbb{R}^{N\times N}$ by the convolution theorem~\cite{convolution}:
\begin{equation}
\label{convolution definition}
    \bm{\kappa}*_\mathcal{G}\bm{X}=\mathcal{F}^{-1}(\mathcal{F}(\bm{\kappa})\cdot\mathcal{F}(\bm{X})) \in\mathbb{R}^{N\times N},
\end{equation}
where $\cdot$ is the matrix multiplication operator, $\mathcal{F}(\cdot)$ and $\mathcal{F}^{-1}(\cdot)$ are the spectral transform (e.g., graph Fourier transform~\cite{bruna2013spectral}) and corresponding inverse transform, respectively. Spectral function $\mathcal{F}(\bm{\kappa})$ is usually parameterized with $\theta$. Let us consider two cases:

\textbf{1) Vector-valued  function.} $\mathcal{F}(\bm{\kappa})=\mathcal{F}_\theta(\bm{\Lambda})$ is parameterized diagonally, where diagonal elements are adjustments on the spectrum of the graph $\mathcal{G}$. Bruna et al.~\cite{bruna2013spectral} directly set $\mathcal{F}_\theta(\bm{\Lambda})=\textrm{diag}(\theta)$, fully free to optimize. ChebNet~\cite{chebnet} further sets $\mathcal{F}_\theta(\bm{\Lambda})=\sum_k\theta_kT_k(\Lambda)$, where $T_k(\cdot)$ is the $k$-th term of Chebyshev polynomials. Most spectral graph neural networks adhere to learning spectral functions as a linear combination of basis functions derived from the graph spectrum, s.a. CayleyNet~\cite{levie2018cayleynets}.


\textbf{2) Matrix-valued  function.} If $\bm{\kappa}$ is parameterized as an matrix-valued kernel, then Eq.~\eqref{convolution definition} is the formula of shift-invariant Transformers~\cite{fno}. Specifically, the vanilla Transformer~\cite{va_trans} is given as:
\begin{equation}
\label{general}
\bm{H}^{(l+1)}=\textrm{softmax}\left(\frac{\bm{H}^{(l)}\bm{W}_q(\bm{H}^{(l)}\bm{W}_k)^\top}{\sqrt{d}}\right)\bm{H}^{(l)}\bm{W}_v,
\end{equation}
where $\bm{H}^{(l)}, \bm{H}^{(l+1)}\in\mathbb{R}^{N\times d}$ are node embeddings from $l$-th and ($l+1$)-th layers, and $\{\bm{W}_q, \bm{W}_k, \bm{W}_v\}\in\mathbb{R}^{d\times d}$ are the query, key, and value learnable matrices. Viewing the Transformer through the kernel technique, the attention matrix can be regarded as an asymmetric, shift-invariant kernel denoted as $R_\theta\in\mathbb{R}^{N\times d\times d}$~\cite{tsai2019transformer, fno}. Then, the spectral function of Eq.~\eqref{general} is:
\begin{equation}
\label{fnofno}
    \bm{H}^{(l+1)}=\mathcal{F}^{-1}(R_\theta\cdot\mathcal{F}(\bm{H}^{(l)}))\in\mathbb{R}^{N\times d},
\end{equation}
where $R_\theta$ is fully parameterized as a neural network. The corresponding derivations are given in Appendix~\ref{relation}.

As shown above, graph convolution relates spectral graph neural networks~\cite{bruna2013spectral}, and (graph) Transformers~\cite{va_trans}. See Appendix~\ref{related work} for details.

\subsection{Wavelet-based Graph Convolution}
To design a new convolution operation, two critical choices must be considered in Eq.~\eqref{convolution definition}: 1) the selection of the transform $\mathcal{F}$ and 2) the parameterization of the kernel $\bm{\kappa}$.

First, the spectral transform $\mathcal{F}$ and its inverse $\mathcal{F}^{-1}$ can be tailored to the specific nature of data. For set data, the Dirac Delta function~\cite{oppenheim1997signals} is employed, while the fast Fourier Transform (FFT) proves efficient for both sequences~\cite{fno} and grids~\cite{afno}. In the context of graphs, the Fourier transform ($\mathcal{F}\rightarrow\bm{U}^\top$) and wavelet transform ($\mathcal{F}\rightarrow\Phi/\Psi_{s_j}$) emerge as two classical candidates. Notably, wavelet transform offers enhanced expressiveness compared to Fourier transform, and this can be attributed to the following reasons: 

\textbf{$\bullet$ Localization in the spatial domain.} Wavelet bases exhibit strong spatial localization~\cite{gw}. Each wavelet corresponds to a signal diffused away from a central node~\cite{gwnn}, enabling the description of specific signal distributions for individual target nodes. In contrast, Fourier bases describe signal changes over the entire graph rather than offering node-specific information. 

\textbf{$\bullet$ Multiple resolutions.} The use of different spatial scales $s_j$ allows the construction of graph wavelet bases with varying receptive fields, which enables the simultaneous fusion of short- and long-range information. Standard graph Fourier bases, represented by fixed eigenvectors $\bm{U}^\top$, maintain a constant resolution. 

\textbf{$\bullet$ Adaptability.} Graph wavelets offer the flexibility to adjust the shapes of unit wavelet bases $g(\cdot)$ and scaling function bases $h(\cdot)$. This adaptability allows for the alignment of basis characteristics with different datasets, potentially enhancing generalization performance. Fourier transform, represented by the fixed basis $\bm{U}^\top$, lacks this adaptability across diverse datasets.

Based on these rich properties, we will utilize SGWT to define the spectral transform in Eq.~\eqref{convolution definition}. Provided that we have $J$ wavelet bases $\{\Psi_{s_j}\}_{j=1}^J$ and one scaling function basis $\Phi$, $\mathcal{F}: \mathbb{R}^{N\times d}\rightarrow \mathbb{R}^{N(J+1)\times d}$ is the stack of transforms from each component as follows:
\begin{equation}
\begin{aligned}
\label{f}
    \mathcal{F}(\bm{H}^{(l)})&=\bm{T}\bm{H}^{(l)}\in\mathbb{R}^{N(J+1)\times d}\\
    &=((\Phi\bm{H}^{(l)})^\top|| (\Psi_{s_1}\bm{H}^{(l)})^\top||...||(\Psi_{s_J}\bm{H}^{(l)})^\top)^\top,
\end{aligned}
\end{equation}
where $\bm{T}=(\Phi^\top|| \Psi_{s_1}^\top||...||\Psi_{s_J}^\top)^\top$ is the overall transform and $||$ means concatenation. Since $\bm{T}$ is not a square matrix, so $\mathcal{F}^{-1}$ should be its pseudo-inverse as $(\bm{T}^\top\bm{T})^{-1}\bm{T}^\top$, where $\bm{T}^\top\bm{T}=\Phi\Phi^\top+\sum_{j=1}^J \Psi_{s_j}\Psi_{s_j}^\top=\bm{U}[h(\lambda)^2+\sum_{j=1}^Jg(s_j\lambda)^2]\bm{U}^\top$. For simplification, we can impose $\bm{T}$ to be tight frames, then $h(\lambda)^2+\sum_{j=1}^Jg(s_j\lambda)^2=\bm{I}$~\cite{leonardi2013tight}, and $\bm{T}^\top\bm{T}=\bm{U}\bm{I}\bm{U}^\top=\bm{I}$. In this case, $\mathcal{F}^{-1}=(\bm{T}^\top\bm{T})^{-1}\bm{T}^\top=\bm{T}^\top$, and Eq.~\eqref{convolution definition} will become:
\begin{equation}
\begin{aligned}
    \bm{H}&^{(l+1)}=\bm{T}^\top(\mathcal{F}(\bm{\kappa})\cdot\bm{T}\bm{H}^{(l)})\in\mathbb{R}^{N(J+1)\times d}\\
    &=(\Phi^\top|| \Psi_{s_1}^\top||...||\Psi_{s_J}^\top)((\mathcal{F}_0(\bm{\kappa})\cdot\Phi\bm{H}^{(l)})^\top||
    \\&\quad(\mathcal{F}_1(\bm{\kappa})\cdot\Psi_{s_1}\bm{H}^{(l)})^\top||
    ...||(\mathcal{F}_J(\bm{\kappa})\cdot\Psi_{s_J}\bm{H}^{(l)})^\top)^\top\\
    &=\Phi(\mathcal{F}_0(\bm{\kappa})\cdot\Phi\bm{H}^{(l)})+\sum_{j=1}^J\Psi_{s_j}(\mathcal{F}_j(\bm{\kappa})\cdot\Psi_{s_j}\bm{H}^{(l)}),
\end{aligned}
\end{equation}
where we separate $\mathcal{F}(\bm{\kappa})$ into several parts $\{\mathcal{F}_j(\bm{\kappa})\}_{j=0}^J$, each of which is assigned to a transform component. To imitate the multi-head attention function~\cite{va_trans}, we choose to concatenate components rather than sum them to get $\bm{H}^{(l+1)}\in\mathbb{R}^{N\times d}$:
\begin{equation}
\begin{aligned}
    \label{final_1}
    &\bm{H}^{(l+1)}=\textrm{MLP}\left(\Phi(\mathcal{F}_0(\bm{\kappa})\cdot\Phi\bm{H}^{(l)})||\right.\\
    &\left.
    \Psi_{s_1}(\mathcal{F}_1(\bm{\kappa})\cdot\Psi_{s_1}\bm{H}^{(l)})||\dots||\Psi_{s_J}(\mathcal{F}_J(\bm{\kappa})\cdot\Psi_{s_J}\bm{H}^{(l)})\right),
\end{aligned}
\end{equation}
where an outermost $\textrm{MLP}$ increases the flexibility. 


Second, we turn to the parameterization of the spectral kernel $\mathcal{F}(\bm{\kappa})$. Here, we express $\mathcal{F}(\bm{\kappa})$ in a matrix-valued form to achieve a more powerful kernel, but with more parameters involved. In Eq.\eqref{fnofno}, the convolution expression is provided under this formulation. Notably, the number of parameters in $R_\theta^{N\times d\times d}$ is quite important, particularly for large-scale graphs with a large value of $N$. To efficiently model $R_\theta$, we adopt parameter sharing among all frequency modes, employing only one Multi-Layer Perceptron (MLP). This results in a significant reduction of parameters in $R_\theta$ from $N\times d\times d$ to $d\times d$. Eq.~\eqref{fnofno} becomes:
\begin{equation}
\label{final_2}
    \bm{H}^{(l+1)}=\mathcal{F}^{-1}(\sigma(\mathcal{F}(\bm{H}^{(l)})\bm{W}_\kappa^{(l)}))\in\mathbb{R}^{N\times d},
\end{equation}
where $\bm{W}_\kappa^{(l)}$ contains learnable weight and bias for neural network $\mathcal{F}(\kappa)$ at $l$-th layer, and $\sigma$ is the activation function. This approach allows various frequency modes to interact, allowing them to collaboratively determine the optimal signal filtering strategy. An alternative method is presented in AFNO~\cite{afno}, introducing a weight-sharing technique that offers improved computational efficiency but with a more intricate design. Finally, combining Eq.~\eqref{final_1} and~\eqref{final_2}, we obtain our  model \M, i.e. a new implementation of graph convolution operation based on wavelets:
\begin{equation}
\begin{aligned}
    \label{final}
    \bm{H}^{(l+1)}=&\textrm{MLP}(\Phi\sigma(\Phi\bm{H}^{(l)}\bm{W}_0^{(l)})||\Psi_{s_1}\sigma(\Psi_{s_1}\bm{H}^{(l)}\bm{W}_1^{(l)})||\\
&\dots||\Psi_{s_J}\sigma(\Psi_{s_J}\bm{H}^{(l)}\bm{W}_J^{(l)}))\in\mathbb{R}^{N\times d},
\end{aligned}
\end{equation}
By its design, \M\ can handle various node interaction ranges, leveraging the multi-resolution feature of graph wavelets, which is similar to traditional Transformers interacting over the whole graph. However, Eq.~\eqref{final} explicitly disentangle the information from different interaction ranges so that the model can adaptively learn which range must be emphasized, whereas traditional Transformers mix short- and long-range information together without distinction. Thus, \M\ surpasses Transformers in controlling distance based information.



\subsection{Theoretical Analysis}
In this section, we demonstrate the effectiveness of the proposed \M\ in capturing both short- and long-range information. Intuitively, a model's ability to integrate global information enables the reception and mixing of messages from distant nodes. Conversely, a model with a limited receptive field can only effectively mix local messages. Hence, assessing the degree of information `mixing' becomes a key property. For this reason, we focus on the concept of \textit{maximal mixing}, defined as follows:
\begin{definition}
\textbf{(Maximal mixing)}~\cite{how}.
    \textit{For a twice differentiable graph-function $y_G$ of node features $\bm{x}_i$, the maximal mixing induced by $y_G$ among the features $\bm{x}_a$ and $\bm{x}_b$ associated with nodes $a, b$ is}
    \begin{equation}
    \label{definition}
        \text{mix}_{y_G}(a, b)=\max\limits_{\bm{x}_i}\max\limits_{1\leq\alpha, \beta\leq d}\left|\frac{\partial^2y_G(\bm{X})}{\partial x_a^\alpha\partial x_b^\beta}\right|.
    \end{equation}
\end{definition}
This definition is established in the context of graph-level task, and $y_G$ is the final output of an end-to-end framework, comprising the primary model and a readout function (e.g., \textrm{mean}, \textrm{max}) applied over the last layer. $\alpha$ and $\beta$ represent two entries of the $d$-dimensional features $\bm{x}_a$ and $\bm{x}_b$.


Next, we employ `maximal mixing' on the proposed \M\, and draw some important results. For simplicity, we only consider one wavelet basis without inverse transform in Eq.~\eqref{final}, i.e. $\sigma(\Psi_{s}\bm{H}^{(l)}\bm{W}_s^{(l)})$. In this equation, we bound the first derivate of non-linear function as $|\sigma'|<c_\sigma$, and set $||\bm{W}_s^{(l)}||\leq w$, where $||\cdot||$ is the operator norm. First, we give an upper bound for each entry in $\Psi_{s}$.
\begin{lemma}[\textbf{Upper bound for graph wavelet}]
\label{aa}
    Let $\Psi=\bm{U}g(\Lambda)\bm{U}^T$. Given a large even number $K>0$, suppose $g$ is $K+1$ times continuously differentiable on [0, 2] and satisfies $g(0)=0, g^{(r)}(0)=0$ for all $r<K$, and $g^{(K)}(0)=C>0$. Then, we have:
    \begin{equation}
        (\Psi_s)_{ij}<\left(\alpha(\hat{\bm{A}})^{K/2}s^K\right)_{ij}, \forall i,j\in V\times V,
    \end{equation}
    where $\alpha=\frac{C\cdot2^K(K+1)}{K!}$.
\end{lemma}
The proof is given in Appendix~\ref{proof_aa}. In this lemma, we assume $g$ is smooth enough at $\lambda=0$. For fair comparison with traditional one-hop message passing framework $\sigma(\bm{A}\bm{H}^{(l)}\bm{W}_s^{(l)})$, we just test the flexibility with the similar form $\sigma(\Psi_{s}\bm{H}^{(l)}\bm{W}_s^{(l)})$. In this case, we derive the depth $m_\Psi$ necessary for this wavelet basis $\Psi_{s}$ to induce the amount of mixing $\text{mix}_{y_G}(a, b)$ between two nodes $a$ and $b$.
\begin{theorem}[\textbf{The least depth for mixing}]
\label{bb}
    Given commute time $\tau(a,b)$~\cite{commute} and number of edges $|E|$. If $\Psi_{s}$ generates mixing $\text{mix}_{y_G}(b, a)$, then the number of layers $m_\Psi$ satisfies
    \begin{equation}
    \begin{aligned}
    \label{asfjisfj}
        m_\Psi \geq& \frac{\tau(a,b)}{2K}+\frac{2|E|}{K\sqrt{d_ad_b}}\left[\frac{\text{mix}_{y_G}(b, a)}{\gamma(\alpha^2s^{2K})^{m_\Psi}}-\right.\\
        &\left.\frac{1}{\lambda_1}(\gamma+|1-\lambda^*|^{Km_\Psi+1})\right],
    \end{aligned}
    \end{equation}
    where $d_a$ and $d_b$ are degrees of two nodes, $\gamma=\sqrt{\frac{d_{max}}{d_{min}}}$, and $|1-\lambda^*|=\max_{0<n\leq N-1}|1-\lambda_n|<1$.
\end{theorem}
The proof is given in Appendix~\ref{proof_bb}. In Eq.~\eqref{asfjisfj}, we denote the lower bound or the minimum number of required layers as $L_{m_\Psi}$. Similarly, $L_{m_A}$ means the minimum number of layers to generate the same mixing $\text{mix}_{y_G}(b, a)$ for $\sigma(\bm{A}\bm{H}^{(l)}\bm{W}_s^{(l)})$. Then, relation between $L_{m_\Psi}$ and $L_{m_A}$ is:
\begin{theorem}[\textbf{Short-range and long-range receptive fields}]
\label{cc}
    Given two random nodes $a$ and $b$, if $\sigma(\Psi_{s}\bm{H}^{(l)}\bm{W}_s^{(l)})$ and $\sigma(\bm{A}\bm{H}^{(l)}\bm{W}_s^{(l)})$ generate the same amount of mixing $\text{mix}_{y_G}(b, a)$, then $L_{m_\Psi}$ and $L_{m_A}$ approximately satisfy the following relation when scale $s\rightarrow\infty$:
    \begin{equation}
    \label{infty}
        L_{m_\Psi} \approx \frac{2}{K}L_{m_A}-\frac{2|E|}{K\sqrt{d_ad_b}}\frac{\text{mix}_{y_G}(b, a)}{\gamma}.
    \end{equation}
    Or, if $s\rightarrow0$, the relation becomes:
    \begin{equation}
    \label{zero}
        L_{m_\Psi} \approx \frac{2}{K}L_{m_A}+\frac{2|E|}{K\sqrt{d_ad_b}}\frac{\text{mix}_{y_G}(b, a)}{\gamma}\cdot\frac{1}{(\alpha^2s^{2K})^{m_\Psi}}.
    \end{equation}
\end{theorem}
The proof is provided in Appendix~\ref{proof_cc}. From Eq.\eqref{infty}, we see that if the scale $s$ is exceedingly large, $\Psi_{s}$ will achieve the same degree of node mixing as one-hop message passing but with much less propagation. In other words, a single-layer $\Psi_{s}$ is able to access longer-range information than one-hop message passing. Conversely, if $s$ is extremely small, the second term on the right-hand side of Eq.~\eqref{zero} will be large, requiring $\Psi_{s}$ to propagate more layers to mix nodes. Consequently, $\Psi_{s}$ exclusively receives shorter-range information than one-hop message passing in this scenario. Note that each term in the concatenation in Eq.~\eqref{final} can be seen as a stack of two $\Psi_{s}$. Therefore, the aforementioned short- and long-range characteristics of $\Psi_{s}$ will also be present in \M\ in a nearly quadratic manner.

% In conclusion, we theoretically prove that the proposed \M\ can arbitrarily control the process of capturing local and global information by adjusting the scale $s$. This property surpasses (graph) Transformers, since the latter mix all information together without controllable distinction.

\begin{figure*}[t]
  \centering
  \includegraphics[scale=0.15]{fig/model.png}
    \vspace{-0.25cm}
  \caption{(a) An overview of our proposed \M. (b) An illustration of Chebyshev polynomials before and after the given transform. In this representation, we distinguish odd and even terms, presenting only the first three terms for each.}
  \label{model}
  \vskip -0.15in
\end{figure*}





==> sec/table/ablation.tex <==
\begin{table}[h]
  \Huge
  \caption{Results of the ablation study. \textbf{Bold}: Best.}
  \label{abla}
  \vskip 0.05in
  \centering
  \resizebox{0.4\textwidth}{!}{
  \renewcommand\arraystretch{1.5}
  \begin{tabular}{ccccc}
    \toprule[4pt]
    \multirow{2}*{Variants} & Pf& VOC & Computer& CoraFull\\
    \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
    &AP $\uparrow$&F1 score $\uparrow$&Accuracy $\uparrow$&Accuracy $\uparrow$\\
    \bottomrule
    w/o $h(\lambda)$&56.56&15.69&89.37&63.36\\
    w/o $g(s_j\lambda)$&61.89&	25.51&	89.67&	63.78\\
    w/o tight frame&64.71&27.79&\textbf{89.77}&\textbf{64.74}\\
    \hline
    Meyer (tight)&61.81&28.56&80.54&51.06\\
    Maxicanhat (non-tight)&64.83&28.22&81.05&50.71\\
    \hline
    \textbf{Ours}&\textbf{65.18}&\textbf{29.42}&89.69&63.97\\
    \toprule[4pt]
  \end{tabular}}
  \vskip -0.1in
\end{table}

==> sec/table/all_base.tex <==
\begin{table*}[h]
  \Huge
  \caption{Quantified results on short-range (S) and long-range (L) datasets compared to base models.}
  \label{all_base}
  \vskip 0.05in
  \centering
  \resizebox{\textwidth}{!}{
  \renewcommand\arraystretch{1.2}
  \begin{tabular}{c|ccccc|ccccc}
    \toprule[4pt]
    \multirow{2}*{Model} & CS (S) & Photo (S) & Computer (S) & CoraFull (S) &ogbn-arxiv (S) & VOC (L) & PCQM (L) & COCO (L) & Pf (L) & Ps (L) \\
    \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}\cmidrule(lr){9-9}\cmidrule(lr){10-10}\cmidrule(lr){11-11}
    &Accuracy $\uparrow$&Accuracy $\uparrow$&Accuracy $\uparrow$&Accuracy $\uparrow$&Accuracy $\uparrow$&F1 score $\uparrow$&MRR $\uparrow$&F1 score $\uparrow$&AP $\uparrow$&MAE $\downarrow$\\
    \hline
    Transformer&93.54±0.43&	89.78±0.68&	83.23±0.75&	50.69±1.17&57.55±0.53&26.94±0.98&31.74±0.20&\textbf{26.18±0.31}&63.26±1.26&25.29±0.16\\
    \textbf{w/ \M}&\textbf{94.77±0.30}&	\textbf{93.93±0.62}&	\textbf{89.69±0.66}&	\textbf{63.97±1.49}&\textbf{71.69±0.26}&	\textbf{29.42±0.94}&	\textbf{33.30±0.10}&	25.11±0.25&\textbf{65.18±0.77}&	\textbf{25.04±0.26}\\
    \hline
    SAN&93.82±0.41&	94.92±0.38&	91.31±0.33&	64.15±1.01&70.25±0.26&32.30±0.39&33.50±0.03&25.92±1.58&63.84±1.21&26.83±0.43\\
    \textbf{w/ \M}&\textbf{95.47±0.31}&	\textbf{95.51±0.22}&	\textbf{91.64±0.42}&	\textbf{66.65±0.83}&\textbf{71.98±0.23}&\textbf{33.33±0.91}&\textbf{34.23±0.13}&\textbf{26.06±0.78}&\textbf{64.54±0.37}&\textbf{26.06±0.17}\\
    \hline
    GraphGPS&95.47±0.31	&94.47±0.46	&89.51±0.74	&62.79±0.72&71.45 ± 0.40&37.48±1.09&33.37±0.06&34.12±0.44&65.35±0.41&25.00±0.05\\
    \textbf{w/ \M}&\textbf{95.89±0.34}&	\textbf{95.37±0.44}&	\textbf{91.00±0.48}&	\textbf{69.14±0.78}&\textbf{72.85±0.24}&\textbf{40.24±0.28}&\textbf{34.50±0.02}&\textbf{35.01±0.22}&\textbf{70.10±0.27}&\textbf{24.95±0.07}\\
    \toprule[4pt]
  \end{tabular}}
  \vskip -0.1in
\end{table*}


==> sec/table/graph_base.tex <==
\begin{table}[h]
  \Huge
  \caption{Accuracy results (i.e. \%$\pm\sigma$) on graph-level tasks compared to base models.}
  \label{graph_base}
  \vskip 0.05in
  \centering
  \setlength{\tabcolsep}{6mm}{
  \renewcommand\arraystretch{1.5}
  \begin{tabular}{cccccc}
    \toprule[4pt]
    \multirow{2}*{Model} & VOC & PCQM & COCO & Pf & Ps \\
    \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
    &F1 score $\uparrow$&MRR $\uparrow$&F1 score $\uparrow$&AP $\uparrow$&MAE $\downarrow$\\
    
    \toprule[2pt]
    Transformer&26.94±0.98&31.74±0.20&\textbf{26.18±0.31}&63.26±1.26&25.29±0.16\\
    \textbf{Transformer+\M}&	\textbf{29.42±0.94}&	\textbf{33.30±0.10}&	25.11±0.25&\textbf{65.18±0.77}&	\textbf{25.04±0.26}\\
    \hline
    SAN&32.30±0.39&33.50±0.03&25.92±1.58&63.84±1.21&26.83±0.43\\
    \textbf{SAN+\M}&\textbf{33.33±0.91}&\textbf{34.23±0.13}&\textbf{26.06±0.78}&\textbf{64.54±0.37}&\textbf{26.06±0.17}\\
    \hline
    GraphGPS&37.48±1.09&33.37±0.06&34.12±0.44&65.35±0.41&25.00±0.05\\
    \textbf{GraphGPS+\M}&\textbf{40.24±0.28}&\textbf{34.50±0.02}&\textbf{35.01±0.22}&\textbf{68.45±0.73}&\textbf{24.95±0.07}\\
    \toprule[4pt]
  \end{tabular}}
  \vskip -0.1in
\end{table}

==> sec/table/hete_base.tex <==
\begin{table*}[h]
  \caption{Quantified results (i.e. \%$\pm\sigma$) on heterophily datasets compared to base models.}
  \label{hete_base}
  \vskip 0.05in
  \centering
  \resizebox{0.97\linewidth}{!}{
  \begin{tabular}{ccccccc}
    \toprule[1.2pt]
    Model&Transformer& \textbf{w/ \M} & SAN & \textbf{w/ \M} & GraphGPS & \textbf{w/ \M}\\
    \hline
    Actor (Accuracy $\uparrow$) & 37.63±0.55&\textbf{38.61±0.74}&31.18±1.08&\textbf{33.63±0.82}&36.52±0.56&\textbf{37.40±1.04}\\
    \hline
    Minesweeper (ROC AUC $\uparrow$)&50.75±1.14&\textbf{93.19±1.56}&92.07±0.35&\textbf{93.98±0.60}&94.03±0.42&\textbf{94.81±0.42}\\
    \hline
    Tolokers (ROC AUC $\uparrow$)&74.04±0.53&\textbf{82.81±1.12}&\textbf{83.37±0.55}&82.73±0.98&84.63±0.88&\textbf{85.38±0.52}\\
    \toprule[1.2pt]
  \end{tabular}}
  \vskip -0.1in
\end{table*}


==> sec/table/hete_com.tex <==
\begin{table*}[h]
\small
  \caption{Qualified results (i.e. \%$\pm\sigma$) on heterophily tasks compared to baselines. \textbf{Bold}: Best, \underline{Underline}: Runner-up, `*' Taken from original papers.}
  \label{hete_com}
  \vskip 0.05in
  \centering
  \resizebox{0.97\linewidth}{!}{
  \begin{tabular}{cccccccc}
    \toprule[1.2pt]
    Model&Graphormer&Nodeformer&Spcformer&SGFormer&NAGphormer&Exphormer&\textbf{\M}\\
    \hline
    Actor (Accuracy $\uparrow$) & 36.41±0.49&34.62±0.82&\textbf{41.93±1.04*}&37.90±1.10&35.39±0.80&36.45±1.21&\underline{38.61±0.74}\\
    \hline
    Minesweeper (ROC AUC $\uparrow$)&90.89±0.53&86.71±0.88&89.93±0.41&\underline{94.31±0.41}&88.06±0.43&90.57±0.64&	\textbf{94.81±0.42}\\
    \hline
    Tolokers (ROC AUC $\uparrow$)&82.75±0.88&78.10±1.03&80.42±0.55&84.57±0.70&82.02±0.98&\underline{84.68±0.77}&\textbf{85.38±0.52}\\
    \toprule[1.2pt]
  \end{tabular}}
  \vskip -0.1in
\end{table*}

==> sec/table/hete_data.tex <==
\begin{table*}[h]
  \centering
  \caption{The statistics of the heterophily datasets.}
  \label{statistics_hete}
  \vskip 0.05in
  \begin{tabular}{c|ccccc}
    \toprule[1.2pt]
    Dataset & \# Graphs & \# Nodes & \# Edges & \# Features & \# Classes \\
    \bottomrule
    Actor &1& 7,600& 33,544& 932& 5\\
    Minesweeper&1& 10,000& 39,402& 7& 2\\
    Tolokers&1& 11,758& 519,000& 10& 2\\
    \toprule[1.2pt]
\end{tabular}
\vskip -0.1in
\end{table*}

==> sec/table/node_base.tex <==
\begin{table}[h]
  \Huge
  \caption{Accuracy results (i.e. \%$\pm\sigma$) on node-level tasks compared to base models.}
  \label{node_base}
  \vskip 0.05in
  \centering
  \resizebox{0.45\textwidth}{!}{
  \renewcommand\arraystretch{1.5}
  \begin{tabular}{ccccc}
    \toprule[4pt]
    Datasets & CS & Photo & Computer & CoraFull\\
    \toprule[2pt]
    Transformer	&93.54±0.43&	89.78±0.68&	83.23±0.75&	50.69±1.17\\
    \textbf{Transformer+\M} &\textbf{94.77±0.30}&	\textbf{93.93±0.62}&	\textbf{89.69±0.66}&	\textbf{63.97±1.49}\\
    \hline
    SAN	&93.82±0.41&	94.92±0.38&	91.31±0.33&	64.15±1.01\\
    \textbf{SAN+\M} &\textbf{95.47±0.31}&	\textbf{95.51±0.22}&	\textbf{91.64±0.42}&	\textbf{66.65±0.83}\\
    \hline
    GraphGPS	&95.47±0.31	&94.47±0.46	&89.51±0.74	&62.79±0.72\\
    \textbf{GraphGPS+\M} &\textbf{95.89±0.34}&	\textbf{95.37±0.44}&	\textbf{91.00±0.48}&	\textbf{68.64±0.78}\\
    \toprule[4pt]
  \end{tabular}}
  \vskip -0.1in
\end{table}
